Building Audio-Visual Digital Twins with Smartphones

Digital twins today are almost entirely visual, overlooking acoustics-a core component of spatial realism and interaction. We introduce AV-Twin, the first practical system that constructs editable audio-visual digital twins using only commodity smartphones. AV-Twin combines mobile RIR capture and a visual-assisted acoustic field model to efficiently reconstruct room acoustics. It further recovers per-surface material properties through differentiable acoustic rendering, enabling users to modify materials, geometry, and layout while automatically updating both audio and visuals. Together, these capabilities establish a practical path toward fully modifiable audio-visual digital twins for real-world environments.

==> section/01-intro-v2.tex <==
\section{Introduction}
\label{sec:introduction}


Sound waves do more than transmit voices or music, they embed the acoustic fingerprint of the environments.
As sound waves propagate and interact with surrounding objects through reflection, diffraction, and scattering, they encode information about the geometry and material properties of the environment.
Capturing accurate acoustic representations of real-world environments is essential for immersive AR/VR, telepresence, spatial audio renderings~\cite{sun2021immersive, naef2002spatialized, chen2024hearable, veluri2024look}, architectural acoustic~\cite{milo2020acoustic, manesh2024acoustic, broyles2022design} and emerging machine learning tasks in speech recognition, source separation and multi-modal scene understanding~\cite{chen2024real, tang2022gwa, chen2020soundspaces, chen2022soundspaces, koyama2021meshrir, GTU-RIR, ratnarajah2024av, veluri2024look, chen2024hearable}.
While today's visual digital twins can reconstruct scene appearance with commodity mobile devices like smartphones~\cite{xxx, yyy}, the acoustic counterpart is still out of reach for common users.


\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{figure/illustration/teaser.pdf}
    \caption{
    Acoustic Capture.
    (a) Two users walk in a room with smartphones to measure RIRs while recording synchronizes trajectories and geometry. (b) \name{} reconstructs the acoustic field of the space, revealing how sound would be perceived at any location. (c) \name{} estimates how different objects such as walls, floors, and tables reflect or absorb sound. \textblue{Acoustic Field twins, Acoustic property twins?}}
    \label{fig:teaser}
    \vspace{-10pt}
\end{figure}

In this work, we view this missing capability through the lens of acoustic digital twins, which is a physically grounded model that reproduces how sound travels in the scene and how each surface interact with the environment. 
Constructing such a acoustic digital twin requires two complementary components.
The first one is \emph{Acoustic Field Twin}, which seeks to model how sound propagates across an entire scene. 
The goal is to reconstruct a continuous sound field for the scene.
This enables tasks such as predicting what a listener would hear at a new position, or synthesizing spatial audio for AR/VR as users move through a scene.
The second one is \emph{Acoustic Property Twin}, which aims to recover how different materials in the scene reflect or absorb sound. For instance, drywall and carpet leave distinct acoustic fingerprints. Estimating these properties allows us to interpret the semantic makeup of a space, or even edit acoustic properties to alter how they sound.


Despite its significance, building acoustic digital twins is largely unrealized in practice.
Modeling of acoustic field has been explored mostly in simulations~\cite{chen2020soundspaces, chen2022soundspaces, tang2022gwa, scheibler2018pyroomacoustics}, while real-world measurements require prohibitively sophisticated setups~\cite{chen2024real, GTU-RIR, koyama2021meshrir, liang2023av}. 
Estimation of acoustic properties has been even less explored: reflection coefficients are typically assumed from reference tables rather than estimated from data~\cite{tang2022gwa, chen2020soundspaces, chen2022soundspaces}.
At the root of these limitations is the bottleneck of \emph{room impulse response (RIR) measurement} in real-world environments.
The RIR records how a short acoustic pulse travels from a source to a microphone along all paths.
Just as a wireless channel encodes multipath and materials in RF, an acoustic RIR encodes similar information in acoustics.
Current pipelines for RIR measurement depend on wired speaker (Tx) and microphone (Rx) arrays, motion-capture systems, or motorized rails, costing over \$100k and many hours to measure even a modest space~\cite{chen2024real, GTU-RIR}.
As a result, acoustic digital twins in real-world has remained out of reach for common user.

% Much of the research on room acoustics~\cite{luo2021neural, su2022inras, liang2023neural, ratnarajah2022mesh2ir, ick2025data} relies on simulations or on a handful of pre-collected datasets spanning only a few environments~\cite{liang2023av, lan2024acoustic, chen2024av, bhosale2024av}.

In this paper, we introduce \name{}, the first practical system that enables building acoustic digital twins in real-world environments. 
Fig.~\ref{fig:teaser}(a) shows our mobile solution in action: two users walk through a room with their smartphones to measure RIRs while simultaneously recording their trajectories and room geometry, all within minutes.
From these measurements, \name{} reconstructs an acoustic field twin of the entire space~(Fig.\ref{fig:teaser}(b)), allowing users to hear how sound would be perceived at any location or to place virtual sources and experience their spatial effects.
It further estimates the acoustic properties twin of objects such as walls, floors, and tables~(Fig.\ref{fig:teaser}(c)), enabling scene editing by virtually adding or removing objects and supporting planning of spaces with awareness of how surfaces shape sound.
The design of \name{} requires to address multiple challenges. We next highlight the key components that make \name{} practical and accurate.

\header{Mobile RIR Capture.}
At the foundation of building acoustic digital twin lies the ability to measure RIRs in real-world environments.
This requires precise time synchronization for time-of-flight (ToF) and device locations for spatial grounding. 
Conventional setups achieve this by wiring devices to the same audio interface for synchronization and using motion-capture systems to track device locations, which are bulky and limited to controlled labs.
\name{} replaces this costly infrastructure with a mobile solution on commodity smartphones, overcoming two key challenges.
The first is synchronization. Without a shared clock, simply cross-correlating a received chirp with the transmitted one leaves the RIR shifted in time. 
Network-based synchronization over WiFi or Bluetooth~\cite{miller2001bluetooth, hao2013wizsync, asgarian2021bluesync} is inadequate since they introduce jitters up to hundreds of millisecond, resulting in propagation errors larger than the size of rooms. 
To overcome this, \name{} performs synchronization directly in the acoustic domain. We embed a two-way handshake into the probe signals, so the Tx and Rx exchange chirps, resolve the ToF, and jointly measure RIRs. With the fine sampling resolution of audio hardware (e.g., 48 kHz) and direct access to raw audio samples, this untethered design achieves sub-ms synchronization.
The second challenge is spatial grounding. RIRs are only meaningful when tied to device locations. While prior systems use motion-capture systems~\cite{chen2024real}, \name{} integrates mobile visual SLAM~\cite{labbe2022multi} to track device locations and reconstruct scene geometry.
We further refine this process by handling interference from human users moving in the scene.
Together, these two designs compress bulky lab setups into smartphones, enabling mobile RIR capture in just minutes.



\header{Acoustic Field Twin.}
While mobile RIR capture provides synchronized RIRs and device poses, reconstructing a full acoustic field twin remains challenging.  
The goal is to predict how sound propagates between arbitrary speaker–listener placements, yet conventional approaches require exhaustively measuring all $N\times M$ Tx–Rx pairs.  
Even modest rooms demand thousands of RIRs, and collecting 2k RIRs can exceed 50 hours~\cite{GTU-RIR}, making dense sampling impractical for everyday users.
\name{} replaces this rigid grid-based process with a dynamic trajectory-based capture.  
Users simply walk through the environment while smartphones continuously collect RIRs, naturally covering diverse geometries and multipath conditions.  
A 20-minute walkthrough is sufficient to reconstruct a high-fidelity acoustic field, which is two orders of magnitude more efficient than dense pairing.  
This mobile workflow democratizes acoustic-field acquisition: anyone with two smartphones can map a room’s acoustics in minutes.
To further boost data efficiency, we introduce AVR++, an extension of prior work~\cite{lan2024acoustic} that directly leverages the 3D scene mesh.  
AVR++ explicitly queries points on the mesh surfaces and predicts their re-transmitted signal towards the microphone location.
By targeting only these acoustically meaningful surface points rather than densely sampling the entire volume, AVR++ further reduces the required capture time from 20 mins to 10 mins while maintaining reconstruction quality.  
Its efficient sampling techniques also accelerate the rendering speed from $100$\,ms to $10$\,ms.
Once reconstructed, the acoustic field twin supports applications including novel-view acoustic synthesis for immersive rendering and RIR-based localization.



\header{Acoustic Property Twin.}
While acoustic field twin reconstructs a scene-wide representation of sound propagation, it does not reveal how individual surfaces shape that propagation. 
Acoustic property twin aims to recover material-dependent reflectivity, but doing so from RIRs is inherently challenging: 
each RIR is a superposition of the direct path and numerous reflections, meaning that no single waveform directly exposes the properties of an individual surface.
\name{} addresses this challenge by combining multiple RIRs recorded across the scene.
While each RIR provides partial constraints, combining them together disentangle the contributions of different surfaces. 
To make this tractable, we leverage introduce vision priors into the framework.
We group the visually similar and adjacent surfaces together to share a single material properties. 
This reduce the dimensionality of the estimation problem and enables reliable material-property estimation from a short scan.
On top of this, we design a differentiable acoustic ray-tracing framework that models path delays and magnitudes. 
Material reflectivities and device patterns are treated as parameters, which are optimized so that the synthesized RIRs closely match the measured ones. 
Through this optimization, the complex multipath effects can be factored back into per-material properties.
This capability enables applications such as interactive scene editing and semantic material understanding.

We build an iOS App that runs in real time for user to capture RIRs. 
The App uses built-in microphone/speaker to transmit probe signals and leverages the camera and LiDAR sensor for visual SLAM to recover device trajectories and room geometry.
We benchmark the mobile RIR capture component and achieve an average ToF estimation error of 0.1~ms and a detection rate of 99.6\%. 
For acoustic field twin, we evaluate RIR reconstruction across four environments and demonstrate more than 100× improvement in data collection efficiency compared to traditional methods. Our proposed AVR++ method can further improve the data efficiency by 2x and improve the rendering speed by 10x.
A user study on audio experience shows that 88\% of participants preferring audio rendered from our method over conventional setups. 
In acoustic localization, augmenting with the reconstructed field reduces error by 50\% and achieves sub-meter accuracy (0.45 m). For acoustic property capture, our framework achieves a mean absolute error of 5.6\% in reflection coefficients estimation and correlation coefficient of 0.96 to the fixed measurement setup.



The key contributions of the paper are as follows:
\begin{itemize}[leftmargin=12pt,itemsep=0pt,topsep=-4pt]
\item We present the first practical mobile system for comprehensive acoustic capture in real-world environments.
\item We design a mobile RIR measurement pipeline with acoustic synchronization and visual SLAM.
\item We design an acoustic field capture framework that requires 100x fewer measurements than previous setup.
\item We propose an acoustic model AVR++ that improve the data-efficiency bottleneck of NeRF-style acoustic fields by 2x and improve the rendering speed by 10x.
\item We incorporate vision priors into the acoustic differentiable rendering framework that estimates materials reflectivity from RIRs.
\item We implement \name{} as a real-time iOS App and extensively evaluate it across diverse indoor environments.
\end{itemize}


==> section/01-intro-v3.tex <==
\section{Introduction}
\label{sec:introduction}



Sound waves do more than transmit voices or music, they embed the acoustic fingerprint of the environments.
As sound waves propagate and interact with surrounding objects through reflection, diffraction, and scattering, they encode information about the geometry and material properties of the environment.
Capturing accurate acoustic representations of real-world environments is essential for immersive AR/VR, telepresence, spatial audio renderings~\cite{sun2021immersive, naef2002spatialized, chen2024hearable, veluri2024look}, architectural acoustic~\cite{milo2020acoustic, manesh2024acoustic, broyles2022design} and emerging machine learning tasks in speech recognition, source separation and multi-modal scene understanding~\cite{chen2024real, tang2022gwa, chen2020soundspaces, chen2022soundspaces, koyama2021meshrir, GTU-RIR, ratnarajah2024av, veluri2024look, chen2024hearable}. \mingmin{we should introduce acoustic digital twin in the first paragraph.}


\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{figure/illustration/teaser.pdf}
    \caption{
    Acoustic Capture.
    (a) Two users walk in a room with smartphones to measure RIRs while recording synchronizes trajectories and geometry. (b) \name{} reconstructs the acoustic field of the space, revealing how sound would be perceived at any location. (c) \name{} estimates how different objects such as walls, floors, and tables reflect or absorb sound. \textblue{Acoustic Field twins, Acoustic property twins?}}
    \label{fig:teaser}
    \vspace{-10pt}
\end{figure}


We frame this goal as constructing an \textit{acoustic digital twin}: a physically grounded model that reproduces how sound travels through a space and how each surface shapes that propagation. Building such a twin requires first reconstructing the acoustic field \mingmin{this requirement needs some justification}, which seeks to model how sound propagates across an entire scene. 
The goal \mingmin{which goal} is to reconstruct a continuous sound field for the scene.
This enables tasks such as predicting what a listener would hear at a new position, or synthesizing spatial audio for AR/VR as users move through a scene.
Beyond acoustic field, the acoustic digital twin subsequently \mingmin{feature or requirement} uncover the material properties that give rise to the observed reflections and reverberations. Estimating these properties allows us to interpret the semantic makeup of a space, or even edit acoustic properties to alter how they sound.


The acoustic field is the foundation of any real-world acoustic digital twin. 
In acoustic field reconstruction, it builds a continues mapping to get room impulse response (RIR) of any given speaker/microphone position in the environment. 
The RIR records how a short acoustic pulse travels from a source to a microphone along all paths.
Just as a wireless channel encodes multipath and materials in RF, an acoustic RIR encodes similar information in acoustics.
However, reconstructing acoustic field usually requires a dense set of RIR measurements.
Obtaining such measurements in real environments has remained prohibitively difficult: existing pipelines rely on wired microphone–speaker arrays, motion-capture rigs, or motorized rails~\cite{chen2024real, GTU-RIR, koyama2021meshrir, liang2023av}, costing over \$100k and requiring hours even for modest rooms. 
As a result, much of the research on room acoustics has relied on simulation~\cite{chen2020soundspaces, chen2022soundspaces, tang2022gwa, scheibler2018pyroomacoustics}, leaving real-world acoustic digital twins largely unrealized.
As a result, acoustic digital twins in real-world has remained out of reach for common user.

To overcome this bottleneck \mingmin{the story right now still focus on the mobile RIR}, we introduce \name{}, a pipeline that reconstructs the acoustic field using mobile RIR capture solution and efficient algorithm design.
\textbf{First}, \name{} performs mobile RIR capture through a pair of smartphones. 
Fig.~\ref{fig:teaser}(a) shows our solution in action: two users walk through a room with their smartphones to measure RIRs while simultaneously recording their trajectories and room geometry, all within minutes. 
RIR measurement requires precise time synchronization for time-of-flight (ToF) and device locations for spatial grounding. 
Conventional setups achieve this by wiring devices to the same audio interface for synchronization and using motion-capture systems to track device locations, which are bulky and limited to controlled labs.
\name{} replaces this costly setup with a mobile solution on smartphones with two key designs.
% The first is synchronization. Without a shared clock, simply cross-correlating a received chirp with the transmitted one leaves the RIR shifted in time. 
% Network-based synchronization over WiFi or Bluetooth~\cite{miller2001bluetooth, hao2013wizsync, asgarian2021bluesync} is inadequate since they introduce jitters up to hundreds of millisecond, resulting in propagation errors larger than the size of rooms. 
The first is dual-purpose acoustic signal protocol to get accurate RIR with time synchronization without wired connection.
\name{} performs synchronization directly in the acoustic domain. 
We embed a two-way handshake into the probe signals, so the Tx and Rx exchange chirps, resolve ToF, and jointly measure RIRs. 
With the fine sampling resolution of audio hardware (e.g., 48 kHz) and direct access to raw audio samples, this untethered design achieves sub-ms synchronization.
The second design is on-device visual SLAM. RIRs are only meaningful when tied to device locations. 
While prior systems use motion-capture systems~\cite{chen2024real}, \name{} integrates mobile visual SLAM~\cite{labbe2022multi} to track device locations and reconstruct scene geometry.
We further refine this process by handling interference from human users moving in the scene.
Together, these two designs compress bulky lab setups into smartphones, enabling mobile RIR capture in just minutes.




\textbf{Secondly}, we introduce a dynamic trajectory-based RIR capturing framework.
While mobile RIR capture solution provides synchronized RIRs and device poses, reconstructing a full acoustic field still remains challenging.  
Conventional approaches measure RIRs exhaustively for every Tx–Rx pair on a grid. This dense pairing quickly becomes prohibitive: with $M$ Tx locations and $N$, one must collect $N\times M$ RIRs, resulting in thousands of measurements even in a modest room. Such exhaustive sampling can take more than 50 hours for 2k RIRs~\cite{GTU-RIR}, which is impractical at scale.
We addresses this inefficiency with a dynamic trajectory-based method.
Instead of anchoring devices at fixed grid points, users can simply traverse the environment with smartphones while continuously recording RIRs. 
This motion dramatically expands spatial coverage and exposes diverse multipath propagation, yielding a much richer basis for
reconstruction. 
In practice, a short 20-minute walkthrough suffices to recover the global acoustic field, up to two orders of magnitude more efficient than dense pairing.
This mobile workflow democratizes acoustic-field acquisition: anyone with two smartphones can map a room’s acoustics in minutes.




\textbf{Thirdly}, current acoustic field model are still not light-weight and efficient.
Prior work either lack physical priors~\cite{luo2022learning}, resulting unsatisfying reconstruction quality, or requires comprehensive acoustic ray sampling~\cite{lan2024acoustic} that reduce the efficiency of the model. 
To solve this problem, we introduce acoustic field model AVR++ that can handle both the problems.
This method incorporates acoustic wave propagation into the rendering and also improve both the data and rendering efficiency compared to prior method.
A key design of AVR++ is to leverage the 3D scene mesh scanned from the mobile RIR capture solution.
To render RIR received by a microphone, AVR++ shoot rays from this microphone position until these rays hit any room mesh.
AVR++ queries points on the room mesh that intersect with these rays and then predicts their re-transmitted signal towards the microphone location.
AVR++ then coherently combine all these signals together by applying time delay and amplitude decay that reflects the acoustic wave propagation phenomenon.
Since our method only tartes acoustically meaningful surface points rather than densely sampling the entire volume~\cite{lan2024acoustic}, AVR++ can further reduces the required capture time from 20~mins to 10~mins while maintaining reconstruction quality.  
Its efficient sampling techniques also accelerate the rendering speed from $100$\,ms to $10$\,ms per RIR sample.
Once the acoustic field is reconstructed, the acoustic field supports applications including novel-view acoustic synthesis for immersive rendering and RIR-based localization.


While the reconstructed acoustic field captures how sound propagates throughout the room, it does not reveal why it propagates that way. \mingmin{more formal description} The spatial patterns of reflections and reverberations are governed by the acoustic properties of surfaces.
For instance, drywall, carpet, wood, and glass each leave distinct acoustic signatures.
Achieving a true acoustic digital twin therefore requires going beyond field estimation to also infer the underlying physical material characteristics that generate these propagation behaviors. \mingmin{explain why}
\name{} extends naturally to this finer-grained task of estimating material-dependent acoustic properties of the environment.
However, recovering material properties is inherently challenging:
each RIR is a superposition of the direct path and numerous reflections, meaning that no single waveform directly exposes the properties of an individual surface.
\name{} addresses this challenge by combining multiple RIRs recorded across the scene.
While each RIR provides partial constraints, combining them together disentangle the contributions of different surfaces. 
To make this problem tractable, we incorporate vision priors into the framework. Visually similar and spatially adjacent surfaces like continues white walls and blackboards tend to share similar material properties. 
Grouping them together reduces the dimensionality of the estimation problem and stabilizes learning from short scans.
On top of this, we design a differentiable acoustic ray-tracing framework that models path delays and magnitudes. 
Material reflectivities and device patterns are treated as parameters, which are optimized so that the synthesized RIRs closely match the measured ones. 
Through this optimization, the complex multipath effects can be factored back into per-material properties.
% This capability enables applications such as interactive scene editing and semantic material understanding.
This material-level formulation further supports dynamic scenes: when objects such as chairs or tables move, the acoustic field changes in ways that traditional static field models struggle to capture. 
By explicitly modeling per-surface properties, \name{} allows the acoustic field to be recomputed under edited or reconfigured geometry, making it suitable for interactive editing and physically grounded scene updates.


\mingmin{we probably don't want to start with the iOS app}
We build an iOS App that runs in real time for user to capture RIRs. 
The App uses built-in microphone/speaker to transmit probe signals and leverages the camera and LiDAR sensor for visual SLAM to recover device trajectories and room geometry.
We benchmark the mobile RIR capture component and achieve an average ToF estimation error of 0.1~ms and a detection rate of 99.6\%. 
For acoustic field reconstruction, we evaluate RIR reconstruction across four environments and demonstrate more than 100× improvement in data collection efficiency compared to traditional methods. Our proposed AVR++ method can further improve the data efficiency by 2x and improve the rendering speed by 10x.
A user study on audio experience shows that 88\% of participants preferring audio rendered from our method over conventional setups. 
In acoustic localization, augmenting with the reconstructed field reduces error by 50\% and achieves sub-meter accuracy (0.45 m). For acoustic property capture, our framework achieves a mean absolute error of 5.6\% in reflection coefficients estimation and correlation coefficient of 0.96 to the fixed measurement setup.



The key contributions of the paper are as follows: \mingmin{too many items here}
\begin{itemize}[leftmargin=12pt,itemsep=0pt,topsep=-4pt]
\item We present the first practical mobile system for comprehensive acoustic capture in real-world environments.
\item We design a mobile RIR measurement pipeline with acoustic synchronization and visual SLAM.
\item We design an acoustic field capture framework that requires 100x fewer measurements than previous setup.
\item We propose an acoustic model AVR++ that improve the data-efficiency bottleneck of NeRF-style acoustic fields by 2x and improve the rendering speed by 10x.
\item We incorporate vision priors into the acoustic differentiable rendering framework that estimates materials reflectivity from RIRs.
\item We implement \name{} as a real-time iOS App and extensively evaluate it across diverse indoor environments.
\end{itemize}


==> section/01-intro-v4.tex <==
\section{Introduction}
\label{sec:introduction}

% still missing defination what is the visual digital twins.
% more justification of acoustic digital twin to the acoustic field.
% AVR++ is not a good name.




Visual digital twins have rapidly become accessible and widely used~\cite{xxx, xxx}. 
With only a smartphone, users can capture 3D geometry, reconstruct meshes, and render photorealistic scenes.
Techniques such as visual SLAM~\cite{xxx}, neural scene reconstruction~\cite{xxx}, and depth sensing~\cite{xxx} have made visual digital twins robust, scalable, and mainstream.
However, the acoustic counterpart, i.e., acoustic digital twin~\cite{xxx}, still remains missing for common users.
% Despite substantial progress on visual modeling, we still lack practical tools and systems for capturing how sound propagates through real environments and how materials shape auditory perception.
An acoustic digital twin reconstructs the full sound propagation behavior of a space, including multipath structure and material responses, to reproduce the auditory experience from any listener–source configuration.
Such capabilities are essential for immersive auditory experience in VR/AR and telepresence, spatial audio rendering~\cite{sun2021immersive, naef2002spatialized, chen2024hearable, veluri2024look}, architectural and building acoustics~\cite{milo2020acoustic, manesh2024acoustic, broyles2022design}, and emerging machine learning tasks such as speech recognition, source separation, and multi-modal scene understanding~\cite{chen2024real, tang2022gwa, chen2020soundspaces, chen2022soundspaces, koyama2021meshrir, GTU-RIR, ratnarajah2024av}.

\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{figure/illustration/teaser.pdf}
    \caption{
    Acoustic Capture.
    (a) Two users walk in a room with smartphones to measure RIRs while recording synchronizes trajectories and geometry. (b) \name{} reconstructs the acoustic field of the space, revealing how sound would be perceived at any location. (c) \name{} estimates how different objects such as walls, floors, and tables reflect or absorb sound. \textblue{To revise}}
    \label{fig:teaser}
    \vspace{-10pt}
\end{figure}


Despite the importance of acoustic digital twins, today’s systems fall far short of enabling it.
An acoustic digital twin requires two fundamental capabilities:
(1) acoustic field reconstruction, which models how sound propagates between arbitrary source–listener positions, and
(2) acoustic property estimation, which uncovers how surfaces such as drywall, carpet, wood, and glass reflect and absorb sound.
For acoustic field reconstruction, current pipelines rely on expensive and dedicated hardware setups~\cite{chen2024real, GTU-RIR, koyama2021meshrir, liang2023av}.
Besides, even with the professional hardware, current framework still requires users lots of time to fully reconstruct an acoustic field of a real environment.
% There is no efficient or accessible system that allows everyday users to capture RIRs densely enough to build the acoustic field of a real environment.
As a result, prior work has depended heavily on simulation~\cite{chen2020soundspaces, chen2022soundspaces, tang2022gwa}, leaving real-world field reconstruction largely unexplored.
For acoustic material property estimation, the gap is even larger. 
There is no existing system capable of estimating per-surface acoustic properties in real environments.
Current methods rely on fixed~\cite{xxx, xxx}, calibrated laboratory setups with controlled source and microphone placement, often requiring hours of recording and specialized equipment.
These constraints make material estimation completely impractical for common users and incompatible with mobile scenarios.
Together, these gaps prevent any practical path toward constructing acoustic digital twins in real-world settings.


In this paper, we propose \name{}, the first practical mobile system that enables common users to build acoustic digital twins efficiently using only commodity smartphones.
Our key insight is that while acoustic digital twins are difficult to construct directly, visual digital twins are robust and easily obtainable on mobile devices.
\name{} leverages these visual capabilities to provide the room geometric and device trajectories needed for accurate acoustic digital modeling.
By tightly coupling acoustic digital twin with visual digital twin, \name{} can build a audio-visual digital twin for immersive experience for common user.
Reaching this requires us to tackle several challenges as detailed below.


Acoustic field reconstruction is the first requirement of an acoustic digital twin.
At the basic of this is the room impulse response (RIR), which records how an emitted acoustic pulse travels through the environment, including all reflections and multipath components. 
One must first collect RIR measurement for a room and then reconstruction the acoustic field. 
The first challenge of acoustic field reconstruction is the high equipment cost for RIR collection.
Existing RIR-collection pipelines rely on expensive loudspeaker–microphone arrays, dedicated audio interfaces for precise synchronization, and motion-capture systems for accurate spatial localization~\cite{chen2024real, GTU-RIR, koyama2021meshrir}. These systems are bulky, costly, and limited to controlled laboratory spaces, making acoustic field reconstruction inaccessible for common users.
\name{} removes this hardware barrier by enabling mobile RIR capture using only commodity smartphones. 
As shown in Fig.~\ref{fig:teaser}(a), two users simply walk through a room while their phones emit probe signals and record synchronized RIRs, alongside trajectories and scene geometry.
To achieve accurate RIRs without wired interfaces, \name{} introduces a dual-purpose acoustic probe that embeds a two-way handshake into the transmitted chirps. 
The phones exchange acoustic signals, estimate their round-trip time-of-flight (ToF), and align their sampling clocks directly in the audio domain. With 48 kHz sampling and raw audio access, this achieves sub-millisecond synchronization, eliminating the need for shared hardware clocks.
To replace motion-capture systems, \name{} leverages the visual digital twin constructed on the device via mobile SLAM and depth sensing. 
The visual twin provides globally consistent trajectories and a 3D geometric mesh, which spatially ground each RIR measurement. We further refine SLAM trajectories to mitigate dynamic interference from users moving within the scene.


The second challenge of reconstructing acoustic field is \textit{prohibitive measurement time}.
Even with mobile RIR collection system, reconstructing an acoustic field traditionally requires measuring thousands of Tx–Rx pairs on a dense grid. For example, collecting 2,000 RIRs can take more than 50 hours in prior setups~\cite{GTU-RIR}, making dense sampling fundamentally impractical.
To eliminate this time bottleneck, \name{} introduces a dynamic-trajectory RIR-collection framework. 
Instead of placing devices at fixed grid points, users freely walk through the environment while phones continuously record RIRs. This natural motion samples a wide variety of geometries and multipath conditions, enabling field reconstruction from a short 15–20 minute walkthrough, over 100× more efficient than grid-based capture. This transforms acoustic-field acquisition into an accessible, casual activity.
To further reduce data and compute requirements, \name{} introduces AVR++, a mesh-guided acoustic field renderer that leverages the 3D mesh from the visual digital twin. AVR++ casts rays from each microphone position to the mesh, identifies acoustically meaningful surface points, and predicts their re-transmitted contributions using learned surface responses. 
It then aggregates these contributions with physically grounded time delays and amplitude decay.
By operating only on mesh surface points—rather than densely sampling the entire 3D volume—AVR++ achieves 2× higher data efficiency and 10× faster rendering than NeRF-style acoustic models~\cite{lan2024acoustic}. With dynamic-trajectory capture and AVR++, \name{} reconstructs high-fidelity acoustic fields from minutes of casual scanning.

% Constructing \todo{Need modify} the acoustic field which is a continuous mapping that predicts sound propagation between arbitrary source (Tx) listener (Rx) positions, is the first core requirement of an acoustic digital twin. However, existing pipelines face two major barriers: \textit{high equipment cost and prohibitive measurement time}. Traditional room-acoustic systems rely on expensive microphone–speaker arrays, dedicated audio interfaces, and motion-capture rigs for synchronization and spatial grounding, making them inaccessible outside controlled labs. We address this cost barrier by leveraging ubiquitous smartphones: using a dual-purpose acoustic probe with a built-in two-way synchronization handshake, \name{} measures RIRs directly between phones with sub-millisecond ToF accuracy, while the visual digital twin extracted through mobile SLAM provides accurate device trajectories and 3D geometry to spatially ground each measurement. 
% Even with mobile capture, reconstructing an acoustic field typically requires thousands of densely sampled Tx–Rx pairs, demanding tens of hours with conventional methods. 
% To overcome this time bottleneck, \name{} introduces dynamic-trajectory capture, where users simply walk through the scene while continuously recording RIRs, naturally covering diverse multipath geometries. We further develop AVR++, a mesh-guided acoustic renderer that uses the visual digital twin’s 3D mesh to trace rays from microphones to surfaces and predict re-transmitted signals. By querying only acoustically meaningful surface points instead of densely sampling free space, AVR++ achieves 2× higher data efficiency and 10× faster rendering, enabling accurate acoustic field reconstruction from only minutes of casual user motion.


While the reconstructed acoustic field captures how sound propagates throughout the room, it does not reveal how the geometries and materials shape the acoustic propagation. The spatial patterns of reflections and reverberations are governed by the acoustic properties of surfaces.
For instance, drywall, carpet, wood, and glass each leave distinct acoustic signatures.
Achieving a true acoustic digital twin therefore requires going beyond field estimation to also infer the underlying physical material characteristics that generate these propagation behaviors. 
Because uncovering these properties allow us to manipulate these properties to resynthesize or recreate new acoustic properties.
However, recovering material properties is inherently challenging:
each RIR is a superposition of the direct path and numerous reflections, meaning that no single waveform directly exposes the properties of an individual surface.
\name{} addresses this challenge by combining multiple RIRs recorded across the scene.
While each RIR provides partial constraints, combining them together disentangle the contributions of different surfaces. 
To make this problem tractable, we incorporate vision priors into the framework. Visually similar and spatially adjacent surfaces like continues white walls and blackboards tend to share similar material properties. 
Grouping them together reduces the dimensionality of the estimation problem and stabilizes learning from short scans.
On top of this, we design a differentiable acoustic ray-tracing framework that models path delays and magnitudes. 
Material reflectivities and device patterns are treated as parameters, which are optimized so that the synthesized RIRs closely match the measured ones. 
Through this optimization, the complex multipath effects can be factored back into per-material properties.
This material-level formulation further supports dynamic scenes: when objects such as chairs or tables move, the acoustic field changes in ways that traditional static field models struggle to capture. 
By explicitly modeling per-surface properties, \name{} allows the acoustic field to be recomputed under edited or reconfigured geometry, making it suitable for interactive editing and physically grounded scene updates.


We build a holistic system solution to capture the acoustic digital twins.
For the acoustic field reconstruction, we build an iOS App that runs in real time for user to capture RIRs. 
The App uses built-in microphone/speaker to transmit probe signals and leverages the camera and LiDAR sensor for visual SLAM to recover device trajectories and room geometry.
We benchmark the mobile RIR capture component and achieve an average ToF estimation error of 0.1~ms and a detection rate of 99.6\%. 
For acoustic field reconstruction, we evaluate RIR reconstruction across four environments and demonstrate more than 100× improvement in data collection efficiency compared to traditional methods. Our proposed AVR++ method can further improve the data efficiency by 2x and improve the rendering speed by 10x.
A user study on audio experience shows that 88\% of participants preferring audio rendered from our method over conventional setups. 
In acoustic localization, augmenting with the reconstructed field reduces error by 50\% and achieves sub-meter accuracy (0.45~m).
For acoustic property capture, our framework achieves a mean absolute error of 5.6\% in reflection coefficients estimation and correlation coefficient of 0.96 to the fixed measurement setup. We also demonstrate that we can alter the geometry position and material property to delivery different audio experience.


The key contributions of the paper are as follows:
\begin{itemize}[leftmargin=12pt,itemsep=0pt,topsep=-4pt]
\item We introduce \name{}, the first system that constructs real-world \emph{acoustic digital twins} using only commodity smartphones, producing both acoustic fields and per-material properties.
\item We develop a mobile RIR-collection pipeline that removes the need for specialized hardware, combining acoustic handshake synchronization with visual SLAM for spatially grounded measurements.

\item We present a practical acoustic field reconstruction framework that uses dynamic trajectory capture and visual-scene geometry to achieve 100× fewer measurements time than prior setup.
\item We design AVR++, a mesh-guided acoustic renderer that leverages the visual digital twin to improve data efficiency by 2× and rendering speed by 10× over NeRF-style approaches.
\item We introduce a vision-guided differentiable material-property estimator that recovers per-surface reflectivities and supports scene editing and acoustic manipulation for immersive experiences.
\end{itemize}


==> section/01-intro.tex <==
\section{Introduction}
\label{sec:introduction}


Sound waves do more than transmit voices or music, they embed the acoustic fingerprint of the environments.
As sound waves propagate and interact with surrounding objects through reflection, diffraction, and scattering, they encode information about the geometry and material properties of the environment.
These acoustic signatures are essential for a wide spectrum of applications:
AR/VR, gaming, and telepresence systems rely on them for immersive spatial audio rendering~\cite{sun2021immersive, naef2002spatialized, chen2024hearable, veluri2024look};
architects use them to guide acoustic design and optimization in classrooms, concert halls, and workplaces~\cite{milo2020acoustic, manesh2024acoustic, broyles2022design};
smart home systems can exploit them for adaptive audio control and personalized experience~\cite{suman2022toward, shabbir2025enhancing, xie2021hearfit+}.
Moreover, large-scale room acoustic datasets have become increasingly critical for machine learning research in speech recognition, source separation, and multi-modal scene understanding~\cite{chen2024real, tang2022gwa, chen2020soundspaces, chen2022soundspaces, koyama2021meshrir, GTU-RIR, ratnarajah2024av, veluri2024look, chen2024hearable}.



\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{figure/illustration/teaser.pdf}
    \caption{
    Acoustic Capture.
    (a) Two users walk in a room with smartphones to measure RIRs while recording synchronizes trajectories and geometry. (b) \name{} reconstructs the acoustic field of the space, revealing how sound would be perceived at any location. (c) \name{} estimates how different objects such as walls, floors, and tables reflect or absorb sound.}
    \label{fig:teaser}
    \vspace{-10pt}
\end{figure}

In this work, we define \emph{Acoustic Capture} as the process of recording and reconstructing acoustic signatures from \emph{real-world environments}. We view acoustic capture as a pair of complementary capabilities.
The first one is \emph{acoustic field capture}, which seeks to model how sound propagates across an entire scene. 
The goal is to reconstruct a continuous sound field for the scene.
This enables tasks such as predicting what a listener would hear at a new position, or synthesizing spatial audio for AR/VR as users move through a scene.
The second is \emph{acoustic property capture}, which aims to recover how different materials in the scene reflect or absorb sound. For instance, drywall and carpet leave distinct acoustic fingerprints. Estimating these properties allows us to interpret the semantic makeup of a space, or even edit acoustic properties to alter how they sound.


\textblue{Despite its significance, acoustic capture remains largely unrealized in practice.
Modeling of acoustic field has been explored mostly in simulations~\cite{chen2020soundspaces, chen2022soundspaces, tang2022gwa, scheibler2018pyroomacoustics}, while real-world measurements require prohibitively sophisticated setups~\cite{chen2024real, GTU-RIR, koyama2021meshrir, liang2023av}. 
Estimation of acoustic properties has been even less explored: reflection coefficients are typically assumed from reference tables rather than estimated from data~\cite{tang2022gwa, chen2020soundspaces, chen2022soundspaces}.
At the root of these limitations is the bottleneck of \emph{room impulse response (RIR) measurement} in real-world environments.
The RIR records how a short acoustic pulse travels from a source to a microphone along all paths.
Just as a wireless channel encodes multipath and materials in RF, an acoustic RIR encodes similar information in acoustics.
Current pipelines for RIR measurement depend on wired speaker (Tx) and microphone (Rx) arrays, motion-capture systems, or motorized rails, costing over \$100k and many hours to measure even a modest space~\cite{chen2024real, GTU-RIR}.
As a result, acoustic capture in real-world has remained out of reach for common user. }

% Much of the research on room acoustics~\cite{luo2021neural, su2022inras, liang2023neural, ratnarajah2022mesh2ir, ick2025data} relies on simulations or on a handful of pre-collected datasets spanning only a few environments~\cite{liang2023av, lan2024acoustic, chen2024av, bhosale2024av}.

In this paper, we introduce \name{}, the first practical system that enables comprehensive acoustic capture in real-world environments. 
Fig.~\ref{fig:teaser}(a) shows our mobile solution in action: two users walk through a room with their smartphones to measure RIRs while simultaneously recording their trajectories and room geometry, all within minutes.
From these measurements, \name{} reconstructs an acoustic field of the entire space~(Fig.\ref{fig:teaser}(b)), allowing users to hear how sound would be perceived at any location or to place virtual sources and experience their spatial effects.
It further estimates the acoustic properties of objects such as walls, floors, and tables~(Fig.\ref{fig:teaser}(c)), enabling scene editing by virtually adding or removing objects and supporting planning of spaces with awareness of how surfaces shape sound.

The design of \name{} requires to address multiple challenges inherent to mobile acoustic capture. We next highlight the key components that make \name{} practical and accurate.

\header{Mobile RIR Capture.}
\textblue{At the heart of acoustic capture lies the ability to measure RIRs in real-world environments.
This requires precise time synchronization for time-of-flight (ToF) and device locations for spatial grounding. Conventional setups achieve this by wiring devices to the same audio interface for synchronization and using motion-capture systems to track device locations, which are bulky and limited to controlled labs.
\name{} replaces this costly infrastructure with a mobile solution on commodity smartphones, overcoming two key challenges.
The first is synchronization. Without a shared clock, simply cross-correlating a received chirp with the transmitted one leaves the RIR shifted in time. 
Network-based synchronization over WiFi or Bluetooth~\cite{miller2001bluetooth, hao2013wizsync, asgarian2021bluesync} is inadequate since they introduce jitters up to hundreds of millisecond, resulting in propagation errors larger than the size of rooms. 
To overcome this, \name{} performs synchronization directly in the acoustic domain. We embed a two-way handshake into the probe signals, so the Tx and Rx exchange chirps, resolve the ToF, and jointly measure RIRs. With the fine sampling resolution of audio hardware (e.g., 48 kHz) and direct access to raw audio samples, this untethered design achieves sub-ms synchronization.
The second challenge is spatial grounding. RIRs are only meaningful when tied to device locations. While prior systems use motion-capture systems~\cite{chen2024real}, \name{} integrates mobile visual SLAM~\cite{labbe2022multi} to track device locations and reconstruct scene geometry.
We further refine this process by handling interference from human users moving in the scene.
Together, these two designs compress bulky lab setups into smartphones, enabling mobile RIR capture in just minutes.
}

% {\color{blue}
% \header{Acoustic Field Capture.}
% While mobile RIR capture provides synchronized RIRs with device locations, building a full acoustic representation of a scene is a different challenge.
% The goal of acoustic field capture is to reconstruct how sound would be received for arbitrary speaker/listener placements. 
% Conventional approaches measure RIRs exhaustively for every Tx–Rx grid pairs.
% With $N$ Tx and $M$ Rx locations, one must collect $N \times M$ RIRs, resulting thousands of measurements even in a modest room..
% For example, such exhaustive sampling can take more than 50 hours for 2k RIRs~\cite{GTU-RIR}, making it impractical and prohibitive for common user.
% \name{} addresses this inefficiency with a dynamic trajectory-based method. Instead of anchoring devices at fixed grid, users traverse the environment with smartphones while continuously collecting RIRs.
% This motion dramatically expands spatial coverage and exposes diverse multipath propagation, yielding a much richer basis for reconstruction. 
% In practice, a short 20-minute walkthrough suffices to recover the global acoustic field, up to two orders of magnitude more efficient than dense pairing.
% It fundamentally democratizes acoustic field collection, any user with two smartphones can map a room’s acoustics in minutes, enabling applications that were previously limited to laboratories with controlled hardware setups.
% To further improve data efficiency, we introduce \emph{AVR++} over prior method~\cite{lan2024acoustic}, a neural acoustic model that directly leverages the reconstructed scene mesh.  
% It directly query the points along mesh surfaces to synthesize the re-transmitted signals from them towards the microphone location. We then combine all the signals from these surfaces to render the final impulse response.
% This method can precisely ping-point the valid re-transmitting signal in the environment compared to previous method that requires comprehensive points sampling through out the whole scene.
% As a result, AVR++ requires significantly fewer recorded RIRs to reconstruct the acoustic field, with the required capturing time reduces from 20 minutes to \emph{approximately 10 minutes}, while maintaining high-quality acoustic field reconstruction.
% Besides, it also improves the rendering speed of about 10~ms, improving prior method by 10x, supporting potential real-time rendering capabilities.
% Once reconstructed, the acoustic field unlocks new applications beyond the original measurements. 
% It enables novel-view acoustic synthesis for immersive auditory experiences, predicting RIRs at unmeasured positions so that any dry audio can be rendered as if heard from that location.
% It also supports RIR-based localization: by matching measured RIRs against the reconstructed field, a device can localize itself to sub-meter accuracy with only a single microphone–speaker pair.
% }


{\color{myblue}
\header{Acoustic Field Capture.}
While mobile RIR capture provides synchronized RIRs and device poses, reconstructing a full acoustic field remains challenging.  
The goal is to predict how sound propagates between arbitrary speaker–listener placements, yet conventional approaches require exhaustively measuring all $N\times M$ Tx–Rx pairs.  
Even modest rooms demand thousands of RIRs, and collecting 2k RIRs can exceed 50 hours~\cite{GTU-RIR}, making dense sampling impractical for everyday users.
\name{} replaces this rigid grid-based process with a dynamic trajectory-based capture.  
Users simply walk through the environment while smartphones continuously collect RIRs, naturally covering diverse geometries and multipath conditions.  
A 20-minute walkthrough is sufficient to reconstruct a high-fidelity acoustic field, which is two orders of magnitude more efficient than dense pairing.  
This mobile workflow democratizes acoustic-field acquisition: anyone with two smartphones can map a room’s acoustics in minutes.
To further boost data efficiency, we introduce AVR++, an extension of prior work~\cite{lan2024acoustic} that directly leverages the 3D scene mesh.  
AVR++ explicitly queries points on the mesh surfaces and predicts their re-transmitted signal towards the microphone location.
By targeting only these acoustically meaningful surface points rather than densely sampling the entire volume, AVR++ reduces the required capture time from 20 minutes to about 10 minutes while maintaining reconstruction quality.  
It also accelerates rendering from $100$\,ms to $10$\,ms.
Once reconstructed, the acoustic field supports applications including novel-view acoustic synthesis for immersive rendering and RIR-based localization.
}

\header{Acoustic Property Capture.}
While acoustic field capture reconstructs a scene-wide representation of sound propagation, it does not reveal how individual surfaces shape that propagation. 
Acoustic property capture aims to recover material-dependent reflectivity, but doing so from RIRs is inherently challenging: 
each RIR is a superposition of the direct path and numerous reflections, meaning that no single waveform directly exposes the properties of an individual surface.
\name{} addresses this challenge by combining multiple RIRs recorded across the scene.
\textblue{
While each RIR provides partial constraints, combining them together disentangle the contributions of different surfaces. 
To make this tractable, we also introduce vision priors into the framework. 
We group the visually similar and adjacent surfaces together to share a single material properties. 
This reduce the dimensionality of the estimation problem and enables reliable material-property estimation from a short scan.}
On top of this, we design a differentiable acoustic ray-tracing framework that models path delays and magnitudes. 
Material reflectivity and device patterns are treated as parameters, which are optimized so that the synthesized RIRs closely match the measured ones. 
Through this optimization, the cumulative effects of multipath can be factored back into per-material properties.
This capability enables applications such as interactive scene editing and semantic material understanding.

\textblue{We build an iOS App that runs in real time for user capture RIRs. 
The App uses the built-in microphones and speakers to transmit probe signals and leverages the camera and LiDAR sensor to run visual SLAM for recovering device trajectories and room geometry.
We benchmark the mobile RIR capture component and achieve an average ToF estimation error of 100~us and a detection rate of 99.6\%. 
For acoustic field capture, we evaluate RIR measurements across four environments and demonstrate more than 100× improvement in data collection efficiency compared to traditional methods. Our proposed AVR++ method can further improve the data efficiency by 2x and improve the rendering speed by 10x.
A user study on audio experience shows that 88\% of participants preferring audio rendered from our method over conventional setups. In acoustic localization, augmenting with the reconstructed field reduces error by 50\% and achieves sub-meter accuracy (0.45 m). For acoustic property capture, our framework achieves a mean absolute error of 5.6\% in reflection coefficients estimation and correlation coefficient of 0.96 to the fixed measurement setup.}



The key contributions of the paper are as follows:
\begin{itemize}[leftmargin=12pt,itemsep=0pt,topsep=-4pt]
\item We present the first practical mobile system for comprehensive acoustic capture in real-world environments.
\item We design a mobile RIR measurement pipeline with acoustic synchronization and visual SLAM.
\item \textblue{We design an acoustic field capture framework that requires 100x fewer measurements than previous setup.}
\item \textblue{ We propose an acoustic model AVR++ that improve the data-efficiency bottleneck of NeRF-style acoustic fields by 2x and improve the rendering speed by 10x.}
\item \textblue{We incorporate vision priors into the acoustic differentiable rendering framework that estimates materials reflectivity from RIRs.}
\item We implement \name{} as a real-time iOS App and extensively evaluate it across diverse indoor environments.
\end{itemize}


==> section/04-avcap.tex <==
\section{Audio visual digital twin}

Building a complete audio–visual digital twin requires not only capturing how a room looks, but also how it sounds. While geometry alone describes the visual structure of an environment, reproducing its acoustics demands understanding how sound propagates through that structure.
Our system unifies these two modalities into a single capture and modeling pipeline. 
Using commodity smartphones, we concurrently measure room impulse responses (RIR) as the users walk through the environment and recover precise device trajectory and room geometry via visual SLAM (\S\ref{sec:acoustic_capture_mobile_platform}).
This multimodal dataset anchors each RIR to the accurate 3D pose for microphone and speaker.
Based on this, we introduce the formulation of acoustic field reconstruction(\S\ref{sec:acoustic_field_capture}) that builds a scene-wide acoustic propagation map and we also introduce visual-assisted acoustic volume rendering that leverage the visual digital twin to reconstruct acoustic field efficiently.


\subsection{Mobile RIR Capture}
\label{sec:acoustic_capture_mobile_platform}

% We design a mobile RIR capture solution that turns commodity smartphones .
\todo{Insert a pipeline figure here}
As illustrated in Fig.\ref{fig:mobile_system_pipeline}, the mobile RIR capture system consists of two concurrent pipelines.
The audio pipeline uses the phone’s speakers and microphones to estimate ToF and extract RIRs (\S\ref{sec:acoustic_two_way} and \S\ref{sec:signal_detection}).
The vision pipeline leverages camera and LiDAR to perform SLAM, recovering device trajectories and reconstructing scene geometry (\S\ref{sec:slam}).
Together, these pipelines efficiently capture RIRs along with device positions and room geometry, producing the unified dataset for understanding acoustic field and property in later sections.



\subsubsection{RIR and ToF Measurement}
\label{sec:acoustic_two_way}


An RIR $h(t)$ is a time-domain signal that characterizes how an acoustic channel responds to an impulse. It describes how sound energy emitted by a source arrives at a receiver over time, including the direct path as well as reflections and reverberations from surrounding surfaces. When the transmitter (Tx, i.e., speaker) emits a probe chirp $c(t)$, the receiver (Rx, i.e., microphone) records a signal $x(t) = c(t) \ast h(t)$, i.e., the probe is convolved with the RIR. 
To estimate the unknown $h(t)$, we cross-correlate the received signal $x(t)$, shown in Fig.~\ref{fig:rir_extraction}(a), with the known probe $c(t)$. 
Since $c(t)$ has a sharply peaked auto-correlation that approximates a delta function (Fig.~\ref{fig:rir_extraction}(b)), this operation effectively cancels out the probe and reveals the RIR:
\begin{equation}
x(t) \ast c(t) = h(t) \ast (c(t) \ast c(t)) \approx h(t) \ast \delta(t) = h(t).
\label{eq:correlation}
\end{equation}
The recovered RIR, as shown in Fig.~\ref{fig:rir_extraction}(c), contains a sharp initial peak shifted by ToF, followed by multipath reflections and late reverberations.
However, Eq.~\ref{eq:correlation} assumes that the start time of the probe signal is known. 
In practice, without precise time synchronization between Tx and Rx, the recovered RIR is shifted by an unknown offset.
Resolving this offset is equivalent to determining the ToF between the devices.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figure/illustration/rir_extraction.pdf}
    \caption{Illustration of RIR extraction. (a) The received signal is cross-correlated with the reference chirp. Since (b) chirp's auto-correlation produces a delta-like peak, (c) the resulting output reveals the RIR, which consists of direct path, multipath reflections and late reverberations.}
    \label{fig:rir_extraction}
    \vspace{-10pt}
\end{figure}

\header{Traditional ToF measurement.}
Conventional acoustic measurement setups~\cite{koyama2021meshrir, chen2024real} obtain ToF by wiring speakers and microphones to the same audio interface for tight synchronization. While accurate, this approach is bulky and impractical for mobile devices. A natural alternative is wireless time synchronization (e.g., NTP or WiFi/Bluetooth), but these methods suffer from jitters up to hundreds of ms, resulting in ranging errors larger than the size of the room.
Lower-level network protocols~\cite{lulf2012evaluation, krueckemeier2019synchronization} can achieve finer synchronization, but they require access to high-rate raw RF samples, which are not exposed by mobile OS such as iOS and Android.


\header{Acoustic synchronization with two-way handshake.}
A key insight of \name{} is that, unlike RF synchronization, mobile devices expose raw audio samples at high sampling rates (e.g., 48 kHz). This makes it possible to perform synchronization directly in the acoustic domain, embedding ToF estimation into the same chirp signals used for RIR measurement.
Specifically, with a 48kHz sampling rate, each sample corresponds to $1/48\text{kHz} \approx 21~\mu$s, which represents the theoretical resolution limit for ToF estimation without specialized hardware.


We use a two-way acoustic handshake protocol that embeds synchronization directly into the probe signals, enabling simultaneous RIR extraction and precise ToF estimation.
Unlike prior systems that employ acoustic handshakes solely for ranging~\cite{peng2007beepbeep, lazik2015ultrasonic}, our approach reuses the same probe signals to capture full RIRs while also resolving inter-device ToF.
As illustrated in Fig.~\ref{fig:acoustic_handshake}, both Tx and Rx continuously record audio. 
At $t_{1}$, the Rx emits a chirp $c_1$, which arrives at Tx at $t_{2}$. Upon detection, Tx immediately transmits a response chirp $c_2$ at $t_{3}$, which propagates back and is recorded by Rx at $t_{4}$.
% One issue is that the Tx and Rx clocks are not synchronized, so the ToF cannot be computed directly from $t_2 - t_1$ or $t_4 - t_3$. 
% Instead, we combine the forward and backward delays to cancel the clock offset and calculate ToF as:
We combine the forward and backward delays to cancel the clock offset and calculate ToF as:
\begin{equation}
\text{ToF} = \frac{(t_4 - t_1) - (t_3 - t_2)}{2}.
\end{equation}
This formulation mirrors the principle in network time protocols~\cite{peterson2007computer}, but here it is used to recover the acoustic ToF for RIR measurement.


\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{figure/illustration/acoustic_synchronization.pdf}
    \caption{Illustration of acoustic two-way handshake design to simultaneously record the RIR and determine the correct ToF.}
    \label{fig:acoustic_handshake}
    \vspace{-10pt}
\end{figure}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figure/illustration/click_pop_noise.pdf}
    \caption{Chirp detection pipeline. 
(a) Real-time chirp detection: Tx recording $x_\text{tx}$ is converted to baseband with filters and further down-sampled to suppress noise and accelerate calculation.
This signal is then correlated with chirp $c_1$ in the time-frequency domain for detection.
(b) Chirp arrival time detection: 
Correlate the recording  with the known chirp $c_2$ in the time domain reveals the RIR (right).
We then identify the correct LoS peak (red marker) despite noise and interference. }
\label{fig:signal_detection}
\vspace{-10pt}
\end{figure}


% We first introduce our dual chirp signal design in acoustic two-way handshale for ToF estimation and RIR extraction.
% After that, We detail the on-device chirp detection to enable TX promptly respond to RX device.
% Finally, we describe the chirp arrival time detection for $t_2$ and $t_4$, which serves as the inputs for ToF calculation discussed earlier.

\subsubsection{Chirp Signal Design and Detection}\mbox{}
\label{sec:signal_detection}


\header{Chirp signal design.} To ensure robust performance of the acoustic two-way handshake protocol, there are several considerations in our chirp signal design.
Firstly, chirps $c_1$ and $c_2$ must lie within the smartphone’s hardware limits, which is typically below 20~kHz. 
To avoid inter‐chirp interference, these two chirps should occupy disjoint frequency bands. 
Moreover, chirps must also be designed with wide bandwidth to sharpen the direct-path peak and improve range resolution. 
In addition, since chirp $c_2$ serves for RIR estimation, it should specifically span frequencies covering common sound in daily life as the primary focus of RIR is for listening experience.
 
Based on these, we choose two linear frequency‐modulated continuous‐wave chirps that are robust to noise~\cite{chen2024real, koyama2021meshrir}:
\begin{itemize}[leftmargin=12pt,itemsep=0pt,topsep=0pt]
  \item Chirp 1 $c_1$ (11~kHz–19~kHz). This chirp does not get interrupted by environmental noise that are usually under 8~kHz~\cite{10.1145/3241539.3241575}.
    Its 8 kHz bandwidth also provides centimeter-level range resolution for ToF estimation.
  \item Chirp 2 $c_2$ (50~Hz–9~kHz).
    This chirp does not overlap with $c_1$ and covers most common sound like human speech (<1~kHz) and instrumental tones (<4~kHz).
\end{itemize}

\noindent
Both chirps are set to 0.2~s, chosen as a balance between motion robustness and signal quality for room-scale measurement. 
Within this short duration, the device moves less than 20~cm at normal walking speeds (0.3~m-1~m), ensuring the RIR remains stable and undistorted. 
In contrast, much shorter chirps (tens of milliseconds) used in prior short-range sensing~\cite{10.1145/3241539.3241575} produce low-SNR outputs that are easily corrupted by environmental noise, leading to poor RIR quality.


\header{Real-time on device chirp detection.}
Fast detection of the chirp signal $c_1$ is critical to our design. If the detection latency is high, the response timestamp $t_3$ will be significantly delayed relative to the arrival time $t_2$. 
The long gap between them will accumulate user movement and distort the RIR estimation due to location changes.
As a result, real-time detection is necessary to achieve mobile RIR capture.

To achieve this, we detect $c_1$ in time-frequency domain that is efficient and robust to noise~\cite{luo2021neural}.
We use the correlation coefficient between the received signal $x_\text{tx}$ and chirp $c_1$ for detection.
This correlation coefficient is invariant to distance-dependent attenuation and peaks only when the signal $x_\text{tx}$ truly matches $c_1$.
This time-frequency based method supports streaming detection to improve efficiency, where only the newly appended audio are transformed with Fast Fourier Transform (FFT).
We also down sample the signal to further improve efficiency.
These operations together reduce the detection latency from $1.1$~s to $0.1$~s, achieving a 90\% reduction over a normal time-domain based detection.
The complete detection process is illustrated in Fig.~\ref{fig:signal_detection}(a).

\header{Chirp arrival time detection.} 
An accurate determination of the chirp arrival time ($t_2$ and $t_4$) must locate the timestamp for the direct path, rather than locating at multipath echo or interference (middle of Fig.~\ref{fig:signal_detection}(b)).
To address this, we develop a robust direct-path detection method and demonstrate it using the detection of $t_4$ as an example.
We first cross-correlate the recording $x_\text{rx}(t)$ with  $c_2(t)$, producing output $h(t)$.
We then find all candidate peaks above a predefined threshold $h_{\min}: \mathcal{P}=\{p_k\!:\!h(p_k)>h_{\min}\}.$
These peaks mark the potential regions of the direct path.
We then scan \(\mathcal{P}\) in ascending order.
For each candidate \(p_k\), we test whether there is a later peak candidate \(p_{k+1}\le p_k+\Delta T\) such that $h(p_{k+1})\ge ah(p_k)$, where $\Delta T$ is a short time window and $a$ is a growth rate ratio.
This tests whether there is a sharp increase in the correlation output that marks the direct path of RIR. 
Once a candidate peak passes the test, the arrival time $t_4$ is determined as the timestamp of the local maximum within the window:
$t_4 = \argmax_{t \in [p_k,\, p_k + \Delta T]}h(t).$
As shown in Fig.~\ref{fig:signal_detection}(b), this method is robust to interference or the false peak caused by multipath.



 \begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figure/illustration/human_masking.pdf}
    \caption{Post processing for SLAM. (a) YOLO-based segmentation and masking of human regions to mitigate their impact on the recovered room geometry. (b) Merging the Tx/Rx scanning. }
    \label{fig:human_mask}
    \vspace{-10pt}
\end{figure}


\subsubsection{Visual digital twin with mobile SLAM}
\label{sec:slam}
While the RIR encodes rich information about acoustic propagation, itself alone is insufficient for building a complete acoustic representation. 
The RIR is only meaningful when tied to device locations and scene geometry.
% Without knowing where the speaker and microphone are located and how the room is shaped, the captured RIRs cannot be contextualized for field reconstruction or localization. 
To this end, we integrate on-device SLAM using built-in camera and LiDAR sensors to jointly capture the visual digital twin that contains device trajectories and scene structure during the scanning. 
This method helps get rid of the cumbersome setup that requires extra and expensive hardware like motion capture system for localizations.
It also transforms acoustic capture from a single-modality process into a multi-modal recording pipeline with both audio and vision data.

\header{SLAM for localization and scene reconstruction.}
We integrate a lightweight vision SLAM algorithm, RTAB-Map~\cite{labbe2022multi}, into our mobile platform and deploy it on both the Tx and Rx devices. The SLAM pipeline uses RGB and LiDAR sensor data to estimate device trajectories, yielding the speaker and microphone positions ($p_\text{tx}$, $p_\text{rx}$) and orientations ($\omega_\text{tx}$, $\omega_\text{rx}$).
In addition to device poses, the SLAM output also provides room geometry $G$, represented as a triangular mesh.


\header{Handling human interference.} Since our system involves two users freely scanning the scene with handheld devices, human bodies are frequently captured in both camera images and LiDAR scans, which corrupts the reconstructed scene (Left of Fig.~\ref{fig:human_mask}(a)).
To mitigate this, we record all sensor streams and perform post-processing with a YOLO based object segmentation model~\cite{wang2024yolov10}.
As shown in the right of Fig.~\ref{fig:human_mask}(a), human regions are masked out in RGB image, which helps remove artifacts and produce a clean environmental reconstruction.


\header{Aligning Tx/Rx coordinates.} RIR measurement requires that Tx and Rx devices share a common coordinate to precisely reflects the delay and attenuation effects of acoustic path.
However, they have individual SLAM scanning and their coordinates are not aligned (left of Fig.~\ref{fig:human_mask}(b)).
To align their coordinates, we reload both database of Tx and Rx and merge them to build a unified pose graph via global loop-closure detection. 
For each matched Tx–Rx frame pair, 2D feature matches are back-projected into 3D using the associated depth maps and camera's intrinsic parameters. 
An inter-session transform is then estimated with random sample consensus (RANSAC) algorithm.
The resulted transform is inserted into global pose graph as an inter-session loop-closure constraint.
Finally, the combined graph is optimized by the general graph optimization (g2o) to jointly refine all poses and produce Tx and Rx coordinates that align with each other. 
As shown in Fig.~\ref{fig:human_mask}(b), after merging the scans, both the coordinates of the Tx/Rx devices and room mesh are well aligned.

% \textred{Following this, we obtain precise TX/RX device positions by querying the SLAM pose history and selecting the poses whose timestamps are the closest to the RIR arrival time $t_\text{RIR}$.
% This process combines both audio and vision stream (Fig~\ref{fig:mobile_system_pipeline}) and produce a complete dataset with RIR, device locations and room geometry: 
% $$\{(h(t), p_\text{rx}, p_\text{tx}, \omega_\text{rx}, \omega_\text{tx}, G)\}.$$} \mingmin{do we really need this paragraph?}






==> section/06-evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}
In this section, we first benchmark the performance of mobile RIR capture with ToF estimation, acoustic field capture for novel view acoustic synthesis and acoustic field capture for material estimation in~\S~\ref{subsec:microbenchmarks}. 
We then show applications on acoustic localization, immersive auditory experience, dynamic scene editing and semantic understanding in~\S~\ref{subsec:evaluation_applications}.

\subsection{System performance}
\label{subsec:microbenchmarks}

\subsubsection{Performance of Mobile RIR capture}\mbox{}

\header{Mobile Platform Implementation.} We integrate the acoustic two-way handshake protocol with RTAB-Map into a standalone iOS App.
Our App can run on both iPhone Pro and iPad Pro, and we use an iPhone 15 Pro Max and an iPad Pro (4th generation).
Both devices are equipped with LiDAR sensors near the camera array.
To maximize pose accuracy, RTAB-Map is configured to update at 5~Hz.
For audio, we use the built-in rear microphone for recording and the default loudspeaker for chirp playing. 
Chirp $c_1$ is transmitted once every 2~s, yielding a collection rate of 0.5~Hz.
This transmission interval guarantees that the extracted RIR from the previous chirp $c_2$ is not distorted by subsequent transmitted $c_1$.
Fig.~\ref{fig:hardware_setup} provides an example of deployment and data collection as two users move in the scene.


\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{figure/illustration/hardware.pdf}
    \caption{Left: Deploy mobile RIR capture on commodity mobile devices with built-in sensors; Right: A snapshot of data capturing, each user holds a mobile device and scans the scene.}
    \label{fig:hardware_setup}
    \vspace{-10pt}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{figure/illustration/localization_results.pdf}
    \caption{Evaluation on the ToF estimation. Left: we measure the ToF error which has an average of 100~us. Right: a case study where Rx is moving steadily towards the Tx and the estimated ToF decrease gradually.}
    \label{fig:tof_error}
    \vspace{-10pt}
\end{figure}


\header{ToF estimation error.}
We compute the ground-truth ToF by measuring the distance between the Tx and Rx device with a laser meter and dividing it by the speed of sound.
As shown in the left of Fig.~\ref{fig:tof_error}, the estimation error remains stable and does not introduce much growth with increasing distance.
At a separation of 9~m between Tx/Rx, the average ToF error is 100~us, corresponding to 4~cm ranging error given the speed of sound.
On the right of Fig.~\ref{fig:tof_error}, we present a case study where the Rx device steadily moves toward the fixed Tx device.
The estimated ToF and corresponding distance decrease linearly over time, confirming the consistency of measurement under device movement.

\header{Chirp detection rate.}
We evaluate the reliability of on-device chirp detection in real measurement sessions across varying Tx/Rx distances (1~m to 15~m). 
During a 30-minute scanning session, our system successfully detects the probing chirp $c_1$ with a rate of 99.6\%, indicating that nearly all transmitted signals are correctly identified. 


\header{Power consumption.}
We evaluate the power consumption of the App to understand its practicality for everyday use.
With a fully charged iPhone, it can operate for 3 hours of continuous capture.
This corresponds to scanning around 9 rooms, assuming a session length of 20 minutes per room. 

\header{RIR similarity metrics.} 
We quantify the distance between two RIRs with the following objective metrics:
\begin{itemize}[leftmargin=12pt,itemsep=0pt,topsep=3pt]
\item Reverberation time (T60) measures how well the model captures the decay rate of reverberation characteristics.
\item Clarity (C50) evaluates the proportion of early-arriving energy over the late-arriving energy. 
\item Early Decay Time (EDT) is the time for the first 10 dB of sound decay, focusing on the initial decay rate of the RIR.
% and revealing whether the model characterizes the early decay slope correctly. 
\item Envelope (Env) error measures RIRs' waveform similarities through envelope error.
\item FFT Amplitude (Amp) error quantifies the discrepancies of amplitude in the frequency-domain. 
\item Multi-scale STFT (STFT) error measures the fine-grained spectral-temporal accuracy over multiple time scales.
\end{itemize}
Across all these metrics, lower values indicate the two RIRs are closer. We will use these metrics to evaluate whether human users will influence the RIR capture quality and the performance of acoustic field reconstruction.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{figure/exp/rir_errors.pdf}
    \vspace{-5pt}
    \caption{Impact of human presence on measured RIRs. We compare the RIR distance w/o and w/ human user during collection.}
    \vspace{-15pt}
    \label{fig:rir_error}
\end{figure}

\header{Influence of human presence.}
To quantify whether the user’s body affects RIR capture when holding the smartphones, we directly compare handheld measurements against reference tripod measurements across five indoor scenes. As shown in Fig. \ref{fig:rir_error}, the differences in C50, T60, and EDT remain very small and tightly concentrated around their means: C50 varies by only ~0.3 dB, T60 by ~2\%, and EDT by ~0.003 s. These results indicate that the presence of the human holding the device has negligible impact on measured RIRs, confirming that \name{} is robust under normal user operation.



\subsubsection{Performance of Acoustic Field Reconstruction}\mbox{}

We evaluate the acoustic field capture performance via novel view acoustic synthesis, where we compare the similarity between rendered RIRs from acoustic field and the unseen measured ones.



\header{Experiment setup.} 
We use two different acoustic capture setup to verify the data efficiency of \name{}.
One is our dynamic trajectory method, where each of the Tx and Rx device is held by a moving user.
The user can freely traverse through the scene while capturing RIRs.
In this setup, the recording session lasts approximately 20 minutes, resulting in a total of 600 samples. 
The other setup is anchor-based, consisting of 20 fixed Tx locations and 100–200 Rx positions per location, yielding a total of 2k–3k RIRs.
In this setup, we put the Tx device at a fixed location and let the other user hold Rx device to collect RIRs.
This simulates the traditional RIR measurement setup, where both the speaker and microphone are repositioned many times during collection.
We collect RIR dataset with both setups in four different environments on our campus, containing typical indoor structure such as desks, chair, blackboard, and small objects.
We hold out 10\% of data from both the dynamic-trajectory and anchor-based setups at each scene to form the test set and train each acoustic model on the two remaining datasets (90\%) separately.
Once the training is done, we let the model to synthesize RIRs at unseen testing locations to verify the model performance.
All the trainings are done with one L40 GPU.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figure/exp/acoustic_field_curve_log.pdf}
    \caption{Validation results of different neural acoustic field models trained on 
    dynamic-trajectory datasets versus traditional anchor-based datasets. 
    The x-axis denotes the data collection time (log scale), and the y-axis shows reconstruction error across multiple acoustic metrics.}
    \label{fig:acoustic_field_curve}
    \vspace{-10pt}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.90\linewidth]{figure/exp/wave_visualization.pdf}
    \caption{Examples of synthesized impulse response with different methods. Orange is the model predictions, blue is the ground truth ones.}
    \label{fig:rir_visualization}
\end{figure}

\header{Results.}
Fig.~\ref{fig:acoustic_field_curve} presents the performance of three neural acoustic field models (NAF, AVR and AVR++) when trained on datasets collected via our dynamic-trajectory method versus the traditional anchor-based method. 
The x-axis denotes the time required for dataset collection, while the y-axis shows error across multiple acoustic metrics (C50, EDT, Env, STFT, Amp, T60).
Results consistently demonstrate that dynamic-trajectory method are far more data-efficient. 
For the same acoustic model, training on our 20-minute dynamic-trajectory dataset often achieves comparable or superior performance to training on anchor-based datasets collected over 3000 minutes.
This corresponds to more than 100× reduction in collection time while still producing plausible RIR reconstructions.
This finding highlights that continuous motion supplies more diverse RIR measurements compared to traditional anchor-based method.
Furthermore, training AVR++ with 10 mins data can almost achieve similar performance of AVR when training on 20 mins, further improving the data efficiency.
Fig.~\ref{fig:rir_visualization} shows the visualization of rendered RIRs for each method. AVR++ can render RIR with better alignment to the ground truth ones.
Besides, we also compare the rendering speed of AVR and AVR++ on a L40 GPU.
While AVR takes 100~ms to render a single RIR of 0.3 second, AVR++ can directly query the point along the surface and it only takes 10~ms to output the same RIR, improving the efficiency by 10x.  




\subsubsection{Performance of Acoustic Property Estimation}\mbox{}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figure/exp/material_estimation_results.pdf}
    \caption{Visualization of material estimations. We show top-down view for each scene at different rows. 
    First col: original mesh; Second col: segmented instances are color coded separately;
    Third col: estimated reflection coefficients, blue and red indicate low and high reflectivity, respectively.}
    \label{fig:optimized_material}
    \vspace{-10pt}
\end{figure}

\header{Experiment setup.} 
We build differentiable acoustic ray tracing on top of the Sionna ray tracing engine~\cite{hoydis2022sionna}.
We adjust the wave speed to match sound propagation and enumerate specular reflections up to eight bounces.
Each segmented surface is associated with a sets of learnable reflection coefficient $Rs$ at frequency of 125, 250, 500, 1k, 2k, 4k, 8k. The rest frequency response are linearly interpolated from these points.
Tx/Rx gain pattern is parameterized by a set of spherical harmonics.
We evaluate this framework on four indoor environments collected by our mobile system.
The geometry and speaker/microphone positions are fixed and not subject to optimization.
All the optimizations are done with one RTX 4070 GPU.


\header{Ground truth measurement.}
To obtain reference reflections for evaluation, we perform controlled measurements using co-located Tx/Rx pair positioned 80\,cm from each surface.  
A broad band chirp signal is emitted toward the surface, and the reflected signal is recorded.  
From each recording, we isolate the reflected component and normalize it by a constant factor to produce a relative reflection measurement.  
Though this value is not an absolute reflection coefficient, it provides a consistent reference across surfaces.  
We can use this measurement to assess whether our estimated coefficients are linearly correlated with the fixed setup. We show the setup and the process to get the second reflection at Fig.~\ref{fig:material_setup}.




\begin{figure}
    \centering
    \includegraphics[width=0.99\linewidth]{figure/exp/reflection_coefficients.pdf}
    \caption{Comparison of estimated reflection coefficient and reference one for each material across different frequency.}
    \vspace{-10pt}
    \label{fig:reflection_coefficient}
\end{figure}

\begin{figure}[t]
  \centering
  \small
    \begin{minipage}[c]{0.55\linewidth}
      \centering
      \includegraphics[width=\linewidth]{figure/illustration/detect_setup.pdf}
      \caption{Experiment setup to get the ground truth reference measurement.}
      \label{fig:material_setup}
    \end{minipage}\hfill
    \begin{minipage}[c]{0.43\linewidth}
      \centering
      \captionof{table}{Results on material reflection coefficients estimations.}
      \begin{adjustbox}{max width=\linewidth}
        \begin{tabular}{ccc}
          \toprule
          Material & Fixed setup & Estimated \\ \midrule
          Drywall & 0.90 & 0.93 \\
          Glass   & 0.88 & 0.92 \\
          Metal   & 1.00 & 0.94 \\
          Wood    & 0.81 & 0.88 \\
          Carpet  & 0.71 & 0.85 \\ \midrule
        \end{tabular}
      \end{adjustbox}
      \label{tab:material_estimations_results}
    \end{minipage}
  \vspace{-10pt}
\end{figure}



\header{Results.} 
Fig.~\ref{fig:optimized_material} shows the textured mesh, segmented mesh and the estimated reflection coefficient (averaged across all frequency).
Across all four rooms, the estimated reflectivity aligns with prior reports.
Enclosure walls (drywall) are consistently the most reflective; floors with carpeting appear substantially less reflective than surrounding walls; and movable furniture, such as tables and chairs that are made of wood, tend to exhibit lower reflectivity.
Fig.~\ref{fig:reflection_coefficient} shows the estimated reflection coefficient compared with the reference one~\cite{standard1990standard, jcw_absorption} across four common materials. 
Results show that the estimated coefficients matched very well with the ground truth one, with a mean absolute error of 5.3\%.
% Tab.~\ref{tab:material_estimations_results} quantifies the estimates against reference valuesfor common materials for broadband acoustic reflection coefficients, including drywall, glass, metal, wood and carpet.
% Averaged over all scenes and materials, the mean absolute error of the reflection coefficient is 7.6\%.
Tab.~\ref{tab:material_estimations_results} quantifies the estimates (averaged across different frequency) and the fixed setup measurement results.
The fixed-setup measurements and our estimated ones exhibit a strong Pearson correlation coefficient ($r\!=\!0.96$).
These results indicate that our method reliably recovers material-dependent reflectivity.



\subsection{Applications}
\label{subsec:evaluation_applications}

\subsubsection{Immersive Audio Rendering}\mbox{}

\noindent
One important application for acoustic field capture is to synthesize the immersive audio contents.
Once the acoustic field of a room is captured, we can freely render how a listener would perceive sound while moving through the environment. 
Along any given trajectory the user would experience in the scene, we first associate each receiver pose with its corresponding RIR by querying the trained neural acoustic field model.
A dry source signal (e.g., speech or music) is then convolved with each RIR to generate short audio segments that capture the acoustic effects at that location. 
To avoid audible discontinuities when stitching these segments together, we apply a cross-fade algorithm that smoothly blends overlapping regions between consecutive segments, producing a continuous and natural listening experience. 
At the same time, the trajectory can be used to render synchronized visual frames from the reconstructed mesh, so that both sound and visuals evolve consistently as the user moves through the space. 
This joint audio-visual synthesis provides an immersive reproduction of the scene from arbitrary paths. 
We evaluate the applications on the immersive auditory experience with a perceptual user study.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.88\linewidth]{figure/exp/user_study.pdf}
    \caption{User study. Left: the interface for user study, where each user is asked to watch and listen two video clip and answer the questions to compare the two videos; Right: average user preferences from three videos.}
    \label{fig:user_study}
    \vspace{-14pt}
\end{figure}


\header{User study setup.} 
For each environment, we define a Rx trajectory and use trained acoustic models to synthesize RIRs along the path.
To compare dynamic trajectory method and anchor-based method, we produce RIRs from neural acoustic model that are trained on these two datasets.
Each RIR is convolved with a dry sound track to obtain a wet rendered sound, paired with a time-synchronized video captured from the receiver's viewpoint for spatial context.
We recruit 17 participants and ask them to watch the video with headphones.
Participants listen to the clips and are then asked to compare the clip along three perceptual dimensions: volume consistency, directional cues, and overall quality.

\header{Results.}
Our user study with 17 participants shows that $88\%$ of responses preferred dynamic-trajectory based method over the anchor-based method in terms of overall quality. 
Additionally, $85\%$ of responses indicate that our method outperforms traditional method in sound volume and directional cues.
% We provide a \href{https://youtu.be/0YNIjtNR9Sk}{\textcolor{blue}{demo video}} used in the user study.

\subsubsection{Acoustic Localization}\mbox{}
In the acoustic localization, given an observed RIR $h(t)$ measured by a single speaker–microphone pair, we infer the most probable microphone location $p_\text{rx}$.
In this setup, the speaker is fixed and emits chirp signals, while the microphone moves freely in the environment and records the corresponding RIRs.
Formally, we estimate
\begin{equation}
   \hat{p}_\text{rx} = \arg\max_{p_\text{rx}} Pr(p_\text{rx}; h(t)),
\end{equation}
where $Pr(p_\text{rx}; h(t))$ denotes the likelihood of a candidate microphone location given the measured RIR $h(t)$.

Unlike traditional acoustic localization approaches that rely on multiple microphones or speakers for triangulation, we exploit the diversity of acoustic path that inherently encoded in a single RIR. 
Variations in arrival times and attenuation from various multipath components provide distinctive signatures of the microphone's position.


% \begin{figure}
%     \centering
%     \includegraphics[width=0.9\linewidth]{figure/illustration/localization_network.pdf}
%     \caption{Illustration for acoustic localization model w/ and w/o the acoustic field model. With acoustic field augmentation, the model predicts result that has less uncertainty.}
%     \label{fig:localization_network}
%     \vspace{-10pt}
% \end{figure}

\header{Model design for localization network.}
To localize the microphone, we use a 1D CNN-based neural network ($g$) that takes raw RIR waveform as input and outputs the probability distribution over candidate microphone positions:
\begin{equation}
    g: h(t) \to Pr(p_\text{rx}).
\end{equation}
With ground truth microphone positions, we discretize the space into a grid of candidate locations and assign each grid cell a probability proportional to a Gaussian distribution centered around the ground-truth position.
This produces a smooth location heatmap that serves as the training target.
The network is trained to predict the probability distribution using a cross-entropy loss, encouraging it to assign high probability prediction to regions near the true position.
At inference time, the network outputs a probability heatmap over all location grids and we apply a weighted sum over top 5 most probable locations to determine the final location.

\header{Data augmentation with acoustic field.}
This acoustic localization method can also benefit from the acoustic field.
The acoustic field $f_\theta$ can synthesize additional RIRs at arbitrary Tx/Rx positions, which generates new samples for training the localization network. 
This field-driven augmentation greatly expands the coverage of the training set.
As a result, the localization network with field augmentation can predict more accurate Rx location  (Fig.~\ref{fig:localization_network}).


\header{Experiment setup.} We collect data in three representative environments: a standard classroom ($8m\times10m$), a lecture hall ($7m\times12m$) and an L-shaped room ($8m\times9m$), each furnished with tables, chairs, etc. 
In each room, we fix the Tx at one location and move the Rx throughout the room for 30 minutes, producing 900 RIRs per room. 
Based on these datasets, we train the localization model with two variants: (1) trained with raw RIRs and (2) additional RIRs augmented from acoustic field.
For each room, we split first 80\% of the data for training and rest for testing, which ensures the test positions are not immediate neighbors of training ones. 
For the variant with the field augmentation, we use the same training set to first reconstruct the acoustic field and then synthesize additional 8k RIRs to augment the training.
We evaluate performance in absolute error, i.e. the average L1 distance between predicted and ground-truth positions.
We also add a KNN baseline for comparison.

\begin{figure}[t]
    \centering
    \includegraphics[width=.9\linewidth]{figure/exp/localization_error.pdf}
    \caption{Acoustic localization results. Left: CDFs of localization error. Right: localization error with different training set ratio.}
    \label{fig:localization_result}
    \vspace{-15pt}
\end{figure}

\header{Results.} 
As shown in the left of Fig.~\ref{fig:localization_result}, our 1D CNN-based model can achieve a medium error of 1~m averaged across three rooms, surpassing KNN baseline by about 0.5~m. Acoustic field model can further boost their performance and reduce the localization error to 45~cm for CNN-based model, decreasing the error by 53\%. This shows that augmenting with the acoustic field enables RIR-based localization to reach sub-meter accuracy with a single speaker/microphone pair with only 24 mins (30×0.8) of data collection.
We also ablate the performance with different training set ratio and summarize the results when training set grows from 20\% to 80\%. 
As shown in the right of Fig.~\ref{fig:localization_result}, acoustic field augmentation can boost the performance by a large margin at various ratio.



\vspace{-2pt}
\subsubsection{Dynamic Scene Editing}\mbox{}

\noindent
Our framework enables interactive editing of the acoustic scene and we provide two cases for this capability. 
% Once material-dependent reflection coefficients are estimated, users can directly manipulate these properties to explore new acoustic scenarios. 
One is material editing in Fig.~\ref{fig:scene_editing}(a). 
We fix the Tx/Rx positions and increase the reflectivity of all the surfaces in the environment. 
As a result, the rendered RIR exhibits a longer late tail and the energy decay curve for the RIR flattens.
This indicates a space with stronger reverberation, as reflected by the increased RT60 and EDT values and the decreased C50, since early energy constitutes a smaller fraction of the total after editing.
We show another example of geometry editing in the Fig.~\ref{fig:scene_editing}(b), where several tables are added into the empty room.
The added geometry reduces the number of path between walls and floor and introduces more absorptions.
The re-rendered RIR shows a shorter late tail and more rapidly diminishing reflections and the energy-decay curve also becomes steeper.
Perceptually, the room would sound "tighter" and less echoic.
This aligns with common observation where one can hear more reverberations when clap hand loudly in an empty or unfurnished room.
But once the room is furnished, the echo becomes less obvious.

\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{figure/exp/scene_editings.pdf}
    \caption{Applications on scene editing. (a) We increase the material reflectivity to increase the reverberation time. (b) We add some extra furniture like tables to the original empty room to reduce the echoes.}
    \label{fig:scene_editing}
    \vspace{-15pt}
\end{figure}

\vspace{-2pt}
\subsubsection{Semantic understanding.}\mbox{}
\noindent
We also evaluate the ability to perform semantic classification based on reflection coefficients. 
We adopt a three-level categorization: coefficients greater than 0.9 are labeled as highly reflective, those between 0.80 and 0.9 as moderately reflective, and those below 0.8 as weakly reflective. 
Our method achieves a classification accuracy of 95.8\%.
We emphasize that our goal is not to identify exact material types, since many common surfaces (e.g., marble, metal, glass, and drywall) exhibit similar reflectivity and cluster within the same category. 
This categorization provides an abstraction of room acoustic reflection level. 

